Functional relations, sharp mapping properties and regularization of the X-ray transform on disks of constant curvature

On simple geodesic disks of constant curvature, we derive new functional relations for the geodesic X-ray transform, involving a certain class of elliptic differential operators whose ellipticity degenerates normally at the boundary. We then use these relations to derive sharp mapping properties for the X-ray transform and its corresponding normal operator. Finally, we discuss the possibility of theoretically rigorous regularized inversions for the X-ray transform when defined on such manifolds.

==> preamble.tex <==

\newtheorem{theorem}{Theorem}[]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{assumptions}{Assumptions}[section]
\newtheorem{problem}{Problem}[section]

\def \Bm {\mathbb{B}}
\def \Cm {\mathbb{C}}
\def \Hm {\mathbb{H}}
\def \Imm {\mathbb{I}}
\def \Nm {\mathbb{N}}
\def \Rm {\mathbb{R}}
\def \Sm {\mathbb{S}}
\def \Um {\mathbb{U}}
\def \Xm {\mathbb{X}}
\def \Zm {\mathbb{Z}}

\newcommand      {\bone}        {{ \mathbbm 1}}

\def\A{\mathcal{A}}
\def\B{\mathcal{B}}
\def\C{\mathcal{C}}
\def\D{\mathcal{D}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\H{\mathcal{H}}
\def\I{\mathcal{I}}
\def\J{\mathcal{J}}
\def\K{\mathcal{K}}
\def\L{\mathcal{L}}
\def\M{\mathcal{M}}
\def\O{\mathcal{O}}
\def\P{\mathcal{P}}
\def\SS{\mathcal{S}}
\def\R{\mathcal{R}}
\def\V{\mathcal{V}}

\def\tu{\tilde{u}}

\def\T{\mathbf{T}}
\def\diam{ {{\rm diam}(X)}}
\def\diag{ {\rm diag} }
\newcommand{\Vol}{ \text{Vol }}

\newcommand{\bb}{\mathbf b}
\newcommand{\bc}{\mathbf c}
\newcommand{\bd}{\mathbf d}
\newcommand{\be}{\mathbf e}
\newcommand{\bh}{\mathbf h}
\newcommand{\bk}{\mathbf k}
\newcommand{\bl}{\mathbf l}
\newcommand{\bp}{\mathbf p}
\newcommand{\bq}{\mathbf q}
\newcommand{\bt}{\mathbf t}
\newcommand{\bu}{\mathbf u}
\newcommand{\bv}{\mathbf v}
\newcommand{\bx}{\mathbf x}
\newcommand{\by}{\mathbf y}
\newcommand{\bz}{\mathbf z}
\newcommand{\bD}{\mathbf D}
\newcommand{\bF}{\mathbf F}
\newcommand{\bG}{\mathbf G}
\newcommand{\bH}{\mathbf H}
\newcommand{\bK}{\mathbf K}
\newcommand{\bL}{\mathbf L}
\newcommand{\bP}{\mathbf P}
\newcommand{\bQ}{\mathbf Q}
\newcommand{\bX}{\mathbf X}
\newcommand{\bY}{\mathbf Y}
\newcommand{\bZ}{\mathbf Z}

\newcommand{\hp}{\hat\phi}
\newcommand{\tp}{\tilde\phi}
\newcommand{\ts}{\tilde S}
\newcommand{\tf}{\tilde F}

\renewcommand{\div}{\nabla\cdot}
\newcommand{\tdiv}{\text{div }}
\newcommand{\del}{\overline{\nabla}}

\newcommand{\where}{\quad\text{ where }}
\newcommand{\qandq}{\quad\text{ and }\quad}
\newcommand{\ric}{\text{Ric}}
\newcommand{\scal}{\text{scal}}
\newcommand{\rank}{\text{rank}}

\newcommand{\bfe}{ {\bf e}}
\newcommand{\bff}{ {\bf f}}
\newcommand{\bfg}{ {\bf g}}
\newcommand{\bfi}{ {\bf i}}
\newcommand{\bfj}{ {\bf j}}
\newcommand{\bfk}{ {\bf k}}
\newcommand{\bft}{ {\bf t}}
\newcommand{\bfu}{ {\bf u}}
\newcommand{\bfv}{ {\bf v}}
\newcommand{\bfw}{ {\bf w}}
\newcommand{\bfx}{ {\bf x}}
\newcommand{\bfA}{ {\bf A}}
\newcommand{\bfG}{ {\bf G}}
\newcommand{\bfH}{ {\bf H}}
\newcommand{\bfI}{ {\bf I}}
\newcommand{\bfP}{ {\bf P}}
\newcommand{\bfR}{ {\bf R}}
\newcommand{\bfS}{ {\bf S}}

\newcommand{\alt}{ {\text{Alt}}}
\newcommand{\tr}{ {\text{tr }}}

\newcommand{\wtA} {\widetilde{A}}

\newcommand{\cout}[1]{}
\newcommand{\cin}[1]{#1}

\newcommand{\x}{\mathrm{x}}
\newcommand{\y}{\mathrm{y}}

\newcommand{\mA}{\mathcal{A}}
\newcommand{\mB}{\mathcal{B}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\mN}{\mathcal{N}}

\newcommand{\fc}{{\mathfrak c}}
\newcommand{\h}{\mathfrak h}
\def\d{{ \mathfrak d}}
\newcommand{\mk}{\mathfrak k}
\newcommand{\w}{\mathfrak w}
\newcommand{\mD}{\mathfrak D}

\newcommand{\bzero}{\mathbf 0}
\newcommand{\bGamma}{\boldsymbol\Gamma}
\newcommand{\btheta}{\boldsymbol \theta}
\newcommand{\bchi}{\boldsymbol \chi}
\newcommand{\bnu}{\boldsymbol \nu}
\newcommand{\brho}{\boldsymbol \rho}
\newcommand{\bxi}{\boldsymbol \xi}
\newcommand{\bnabla}{\boldsymbol \nabla}
\newcommand{\bOm}{\boldsymbol \Omega}
\newcommand{\bomega}{\boldsymbol \omega}
\newcommand{\cd}[2]{{#1}\!\cdot\!{#2}}
%\newcommand{\cout}[1]{}
%\newcommand{\cin}[1]{#1}
\newcommand{\sgn}[1]{\,{\rm sign}(#1)}
\newcommand{\bsgn}[1]{\,{\rm sign}\big(#1\big)}
\newcommand{\Bsgn}[1]{\,{\rm sign}\Big(#1\Big)}


\def \supp { {\mbox{supp}}}
\def \dist { {\mbox{dist }}}
\def \st { {|\,}}
\def \sp {\text{sp}}

\newcommand{\da}{\downarrow}
\newcommand{\dprod}[2]{\left\langle{#1},{#2}\right\rangle}
\newcommand{\dbar}{\overline{\partial}}
\newcommand{\zbar}{\overline{z}}

\newcommand{\Phiadj}{-\overline{\Phi}}


\def \i {\boldsymbol\iota}

\newcommand{\mat}[4]{\left[ \begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array} \right]}

\renewcommand{\Im}{\mathbb{I}\mathrm{m} }


%%-- default page dimensions
%\voffset 0.0cm
\hoffset 0.0cm
%\textheight 24cm
\textwidth 16.0cm
%\topmargin -3cm
\oddsidemargin 0.0cm
\evensidemargin 0.0cm



